Modality Influence in Multimodal Machine Learning

Multimodal Machine Learning has emerged as a prominent research direction across various applications such as Sentiment Analysis, Emotion Recognition, Machine Translation, Hate Speech Recognition, and Movie Genre Classification. This approach has shown promising results by utilizing modern deep learning architectures. Despite the achievements made, challenges remain in data representation, alignment techniques, reasoning, generation, and quantification within multimodal learning. Additionally, assumptions about the dominant role of textual modality in decision-making have been made. However, limited investigations have been conducted on the influence of different modalities in Multimodal Machine Learning systems. This paper aims to address this gap by studying the impact of each modality on multimodal learning tasks. The research focuses on verifying presumptions and gaining insights into the usage of different modalities. The main contribution of this work is the proposal of a methodology to determine the effect of each modality on several Multimodal Machine Learning models and datasets from various tasks. Specifically, the study examines Multimodal Sentiment Analysis, Multimodal Emotion Recognition, Multimodal Hate Speech Recognition, and Multimodal Disease Detection. The study objectives include training SOTA MultiModal Machine Learning models with masked modalities to evaluate their impact on performance. Furthermore, the research aims to identify the most influential modality or set of modalities for each task and draw conclusions for diverse multimodal classification tasks. By undertaking these investigations, this research contributes to a better understanding of the role of individual modalities in multi-modal learning and provides valuable insights for future advancements in this field.

==> Tables/dataSet-MT.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Image	& Image & Text   \\\midrule
	BLUE       & 36.75  & 4 & 40 \\\midrule
	METEOR       & 54.95  & 4 &57 \\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets-ER.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
CMU-MOSI\cite{zadeh2018multimodal}	         & & &\\\midrule
IEMOCAP\cite{busso2008iemocap }    & & &\\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets-HateSpeech.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
Hate speech memes \cite{kiela2020hateful }       & & &\\\midrule


\bottomrule
\end{tabular}


==> Tables/datasets-QA.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
CMU-MOSI\cite{zadeh2018multimodal}	       & & &\\\midrule


\bottomrule
\end{tabular}

==> Tables/datasets-SA.tex <==
\begin{tabular}{L{2cm}L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}L{2cm}}
\toprule

 Tasks & Dataset &	Text & Audio	& Video & Available  Pre-processing &  Details\\\midrule
\multirow{2}{*}{}CMU-MOSI\cite{zadeh2016mosi}    & & &\\\midrule
CMU-MOSEI\cite{zadeh2018multimodal }     & 63727 sentence & &90.23h &  16514 videos\\\midrule

\bottomrule
\end{tabular}


==> Tables/datasets-Translation.tex <==
\begin{tabular}{L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}}
\toprule

 Dataset &	Text & Audio	& Video & Available  Pre-processing   \\\midrule
	       & & &\\\midrule


\bottomrule
\end{tabular}

==> Tables/datasets.tex <==
\begin{tabular}{L{2cm}L{2cm}L{1.5cm}L{1.5cm}L{1.5cm}L{4cm}L{2cm}}
\toprule

 Tasks & Dataset &	Text & Audio	& Video & Available  Pre-processing &  Details\\\midrule
\multirow{2}{*}{M-SA}
&CMU-MOSI\cite{zadeh2016mosi}    & & &\\\cline{2-7}
&CMU-MOSEI\cite{zadeh2018multimodal }     & 63727 sentence & &90.23h &  16514 videos\\\midrule
\multirow{2}{*}{ER} &    & & &\\\cline{2-7}
  
 
    &  & & &   \\

\multirow{2}{*}{M-HS} &  Hate Memes   & & &\\\cline{2-7}
  
 
 MMHS150K   & 63727 sentence & &90.23h &  16514 videos\\\midrule

\multirow{2}{*}{M-Movie Class.} &    & & &\\\cline{2-7}
  
 
    &  & & &  \\\midrule

\multirow{2}{*}{M-Translation} &     & & &\\\cline{2-7}
  
 
    &  & & &   \\\midrule
\multirow{2}{*}{Food Class.} &    & & &\\\cline{2-7}
  
 
    &  & & &   \\
\bottomrule
\end{tabular}


==> Tables/ur-funny.tex <==
\begin{tabular}{L{1cm}L{2cm}L{1.6cm}L{2.4cm}}
\toprule

 Mertic &	Text  & Image & Image + text   \\\midrule
	BLUE  &     &    &   39 \\\midrule
	METEOR   &      &    &  56.4 \\\midrule
        $\Delta $\% &     &        & 100\% \\\midrule
 
\bottomrule
\end{tabular}

==> old-ref.tex <==
\bibitem{b1} Al-Shedivat M, Wilson AG, Saatchi Y, Hu Z, Xing EP (2017)
Learning scalable deep Kernels with recurrent structure.
\bibitem{b2} Hofmann T, Schölkopf B, Smola AJ (2008) Kernel methods in
machine learning. Ann Stat 
\bibitem{b3} Nair K.Nikhitha  A.Afzal  S.Asharaf Deep Kernel machines: a survey.  8 June 2019.
\bibitem{b4} Aronszajn N (1950) Theory of reproducing Kernels. Trans Am
Math Soc 
\bibitem{b5} Poria S, Cambria E, Gelbukh A (2015) Deep convolutional neural network textual features and multiple Kernel learning for
utterance-level multimodal sentiment analysis. In: Proceedings
of the 2015 conference on empirical methods in natural language
processing, 

\bibitem{b6} Afzal A, Asharaf S (2018) Deep multiple multilayer Kernel
learning in core vector machines. Expert Syst Appl 96:149–156.
\bibitem{b7} Afzal A, Asharaf S (2017) Deep Kernel learning in core vector
machines. Pattern Anal Appl 21:721

\bibitem{b8} Chen D, Jacob L, Mairal J (2018) Biological sequence modeling with convolutional Kernel networks. bioRxiv p 217257

\bibitem{b9} Shawe-Taylor J, Cristianini N (2004) Kernel methods for pattern
analysis. Cambridge University Press, Cambridge

\bibitem{b10} Charu C. Aggarwal. Neural Networks and Deep Learning. Springer, Cham, 2018

\bibitem{b11} Sutskever I, Hinton G (2010) Temporal-Kernel recurrent neural
networks. Neural Netw 
\bibitem{b12} Slimane Bellaouar. Noyaux de mots et d'arbres : efficacite et unification. PhD thesis,
Universite Amar Telidji-Laghouat, Algerie, 2018. P20

\bibitem{b13} Matthew A. Wright and Joseph E. Gonzalez
Transformers are Deep Infinite-Dimensional Non-Mercer Binary
Kernel Machines
University of California
Berkeley, CA 94705

\bibitem{b14}Marc Peter,Deisenroth, A. Aldo Faisal, Cheng Soon Ong;
MATHEMATICS FOR MACHINE LEARNING by Cambridge University Press 2020

\bibitem{b15}
THOMAS M. COVER, 
Geometrical and Statistical Properties of Systems of
Linear Inequalities with Applications in Pattern
Recognition
\end{thebibliography}

==> transformerTikz.tex <==


\begin{tikzpicture}[scale=0.85]
\definecolor{emb_color}{RGB}{252,224,225}
\definecolor{multi_head_attention_color}{RGB}{252,226,187}
\definecolor{add_norm_color}{RGB}{242,243,193}
\definecolor{ff_color}{RGB}{194,232,247}
\definecolor{softmax_color}{RGB}{203,231,207}
\definecolor{linear_color}{RGB}{220,223,240}
\definecolor{gray_bbox_color}{RGB}{243,243,244}
\draw[fill=gray_bbox_color, line width=0.046875cm, rounded corners=0.300000cm] (-0.975000, 6.455000) -- (2.725000, 6.455000) -- (2.725000, 1.305000) -- (-0.975000, 1.305000) -- cycle;

\draw[line width=0.046875cm, fill=emb_color, rounded corners=0.100000cm] (0.000000, 0.000000) -- (2.500000, 0.000000) -- (2.500000, -0.900000) -- (0.000000, -0.900000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,-0.450000) {Input \vspace{-0.05cm} \linebreak Embedding};m
 
 \draw[line width=0.046875cm, fill=add_norm_color, rounded corners=0.100000cm] (0.000000, 3.730000) -- (2.500000, 3.730000) -- (2.500000,3.180000) -- (0.000000,3.180000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,3.430000) {Add \& Norm};

\draw[line width=0.046875cm, fill=multi_head_attention_color, rounded corners=0.100000cm] (0.000000, 3.030000) -- (2.500000, 3.030000) -- (2.500000, 2.130000) -- (0.000000, 2.130000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,2.580000) {Multi-Head \vspace{-0.05cm} \linebreak Attention};
\draw[line width=0.046875cm] (1.250000, 3.030000) -- (1.250000, 3.180000);
 
 

\draw[line width=0.046875cm] (1.250000, 5.900000) -- (1.250000, 5.730000);

%%%%

\draw[line width=0.046875cm, fill=add_norm_color, rounded corners=0.100000cm] (0.000000, 6.230000) -- (2.500000, 6.230000) -- (2.500000, 5.730000) -- (0.000000, 5.730000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,5.980000) {Add \& Norm};

\draw[line width=0.046875cm, fill=ff_color, rounded corners=0.100000cm] (0.000000, 5.580000) -- (2.500000, 5.580000) -- (2.500000, 4.680000) -- (0.000000, 4.680000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,5.130000) {Feed \vspace{-0.05cm} \linebreak Forward};
 
\draw[line width=0.046875cm, fill=linear_color, rounded corners=0.100000cm] (0.000000, 10.280000) -- (2.500000, 10.280000) -- (2.500000, 9.780000) -- (0.000000, 9.780000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,10.030000) {Linear};
 
\draw[line width=0.046875cm, fill=softmax_color, rounded corners=0.100000cm] (0.000000, 11.380000) -- (2.500000, 11.380000) -- (2.500000, 10.880000) -- (0.000000, 10.880000) -- cycle;
\node[text width=2.500000cm, align=center] at (1.250000,11.130000) {Softmax};
\draw[line width=0.046875cm] (1.250000, 0.600000) circle (0.200000);
\draw[line width=0.046875cm] (1.410000, 0.600000) -- (1.090000, 0.600000);
\draw[line width=0.046875cm] (1.250000, 0.760000) -- (1.250000, 0.440000);
 
\draw[line width=0.046875cm] (0.350000, 0.600000) circle (0.400000);
\draw[line width=0.046875cm] (-0.030000, 0.600000) -- (-0.014490, 0.629156) -- (0.001020, 0.657833) -- (0.016531, 0.685561) -- (0.032041, 0.711884) -- (0.047551, 0.736369) -- (0.063061, 0.758616) -- (0.078571, 0.778258) -- (0.094082, 0.794973) -- (0.109592, 0.808486) -- (0.125102, 0.818576) -- (0.140612, 0.825077) -- (0.156122, 0.827883) -- (0.171633, 0.826946) -- (0.187143, 0.822284) -- (0.202653, 0.813971) -- (0.218163, 0.802145) -- (0.233673, 0.786999) -- (0.249184, 0.768783) -- (0.264694, 0.747796) -- (0.280204, 0.724382) -- (0.295714, 0.698925) -- (0.311224, 0.671845) -- (0.326735, 0.643584) -- (0.342245, 0.614608) -- (0.357755, 0.585392) -- (0.373265, 0.556416) -- (0.388776, 0.528155) -- (0.404286, 0.501075) -- (0.419796, 0.475618) -- (0.435306, 0.452204) -- (0.450816, 0.431217) -- (0.466327, 0.413001) -- (0.481837, 0.397855) -- (0.497347, 0.386029) -- (0.512857, 0.377716) -- (0.528367, 0.373054) -- (0.543878, 0.372117) -- (0.559388, 0.374923) -- (0.574898, 0.381424) -- (0.590408, 0.391514) -- (0.605918, 0.405027) -- (0.621429, 0.421742) -- (0.636939, 0.441384) -- (0.652449, 0.463631) -- (0.667959, 0.488116) -- (0.683469, 0.514439) -- (0.698980, 0.542167) -- (0.714490, 0.570844) -- (0.730000, 0.600000);
 

\draw[line width=0.046875cm, -latex] (1.250000, 3.680000) -- (1.250000, 4.680000);
 

\draw[line width=0.046875cm, -latex] (1.250000, 0.000000) -- (1.250000, 0.400000);
\draw[line width=0.046875cm, -latex] (1.250000, 0.800000) -- (1.250000, 2.130000);
 
\draw[line width=0.046875cm] (0.750000, 0.600000) -- (1.050000, 0.600000);
 
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 4.080000) -- (-0.750000, 4.080000) -- (-0.750000, 5.980000) -- (0.000000, 5.980000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.530000) -- (-0.750000, 1.530000) -- (-0.750000, 3.430000) -- (0.000000, 3.430000);
%\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (5.250000, 1.530000) -- (7.250000, 1.530000) -- (7.250000, 3.830000) -- (6.500000, 3.830000); 

\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.730000) -- (0.312500, 1.730000) -- (0.312500, 2.130000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 1.730000) -- (2.187500, 1.730000) -- (2.187500, 2.130000);

\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 6.230000) -- (1.250000, 7.230000) -- (3.250000, 7.230000) -- (3.250000, 4.680000) -- (4.312500, 4.680000) -- (4.312500, 5.080000);
\draw[-latex, line width=0.046875cm, rounded corners=0.200000cm] (1.250000, 6.230000) -- (1.250000, 7.230000) -- (3.250000, 7.230000) -- (3.250000, 4.680000) -- (5.250000, 4.680000) -- (5.250000, 5.080000);

\draw[line width=0.046875cm, -latex] (1.250000, -1.500000) -- (1.250000, -0.900000);
 
\node[text width=2.500000cm, anchor=north, align=center] at (1.250000,-1.500000) {Inputs};

\node[text width=2.500000cm, anchor=south, align=center] at (1.250000,11.980000) {Output \vspace{-0.05cm} \linebreak Probabilities};
\node[anchor=east] at (-1.175000,3.880000) {$N\times$};

\node[text width=2.000000cm, anchor=east] at (0.250000,0.600000) {Positional \vspace{-0.05cm} \linebreak Encoding};

\end{tikzpicture}
